Crypt$\epsilon$: Crypto-Assisted Differential Privacy on Untrusted Servers

Differential privacy (DP) has steadily become the de-facto standard for achieving privacy in data analysis, which is typically implemented either in the "central" or "local" model. The local model has been more popular for commercial deployments as it does not require a trusted data collector. This increased privacy, however, comes at a cost of utility and algorithmic expressibility as compared to the central model. In this work, we propose, Crypt$\epsilon$, a system and programming framework that (1) achieves the accuracy guarantees and algorithmic expressibility of the central model (2) without any trusted data collector like in the local model. Crypt$\epsilon$ achieves the "best of both worlds" by employing two non-colluding untrusted servers that run DP programs on encrypted data from the data owners. Although straightforward implementations of DP programs using secure computation tools can achieve the above goal theoretically, in practice they are beset with many challenges such as poor performance and tricky security proofs. To this end, Crypt$\epsilon$ allows data analysts to author logical DP programs that are automatically translated to secure protocols that work on encrypted data. These protocols ensure that the untrusted servers learn nothing more than the noisy outputs, thereby guaranteeing DP (for computationally bounded adversaries) for all Crypt$\epsilon$ programs. Crypt$\epsilon$ supports a rich class of DP programs that can be expressed via a small set of transformation and measurement operators followed by arbitrary post-processing. Further, we propose performance optimizations leveraging the fact that the output is noisy. We demonstrate Crypt$\epsilon$'s feasibility for practical DP analysis with extensive empirical evaluations on real datasets.

==> App_diag.tex <==
\section{Additional Experimental Results}
\begin{figure}
     \includegraphics[width=0.5\linewidth]{scale2.pdf}
        \caption{Scalability of \system Programs Cntd.}\label{scale}
    \end{figure}
    \begin{figure}
     \includegraphics[width=0.5\linewidth]{2_final.pdf}
        \caption{Accuracy Analysis of \system Program 2 }\label{scale}
    \end{figure}
    \begin{figure}
     \includegraphics[width=0.5\linewidth]{4_final.pdf}
        \caption{Accuracy Analysis of \system Program 4 }\label{scale}
    \end{figure}
    \begin{figure}
     \includegraphics[width=0.5\linewidth]{6_finals.pdf}
        \caption{Accuracy Analysis of \system Program 6 }\label{scale}
    \end{figure}
\eat{\begin{figure*}
    \begin{subfigure}[b]{0.25\linewidth}
        \centering
        %\includegraphics[width=5cm,height=3.1cm]{t1.pdf}
         \includegraphics[width=1\linewidth]{2_final.pdf}
        \caption{ Program 2}
        \label{fig:P2}
    \end{subfigure}
    \begin{subfigure}[b]{0.25\linewidth}
    \centering \includegraphics[width=1\linewidth]{4_final.pdf}
        \caption{Program 4}
        \label{fig:P4}\end{subfigure}
    \begin{subfigure}[b]{0.25\linewidth}
    \centering    \includegraphics[width=1\linewidth]{6_finals.pdf}
        \caption{Program 6}
        \label{fig:P6}\end{subfigure}
   \caption{Accuracy Analysis of Crypt$\epsilon$ Programs Cntd.}
   \label{accuracy}
\end{figure*}

 
\stitle{Metrics:}\\
\textit{Accuracy}}



==> Program.tex <==
\section{Writing Crypt$\epsilon$ Programs}\label{program}
In this section we illustrate via examples how the aforementioned primitives can be composed into a Crypt$\epsilon$ program to answer data queries.
Crypt$\epsilon$ programs can be classified into three classes based on the number and type of interaction required between the \textsf{AS} and the \textsf{CSP}.  Note that the details about the various interactions for the primitives are explained in the following section under implementations. 
\paragraph{\textbf{Single Decrypt Interaction Programs}}
Recall that the output of all the transformation primitives are encrypted.  Since  the \textsf{CSP} has exclusive access to the secret key, it is the only entity in the Crypt$\epsilon$ setting capable of decryption. Thus for releasing any result (albeit noisy) in the clear, we need to interact at least once with the \textsf{CSP} so that it can decrypt the encrypted noisy answer. Crypt$\epsilon$ supports this type of interactions via the two measurement primitives. Some Crypt$\epsilon$ programs require only this one round of interaction at the very end to release the noisy output. All other transformations can be performed by the \textsf{AS} via homomorphic operations on the encrypted data records. Typically these programs are counting queries on a single attribute or noisy max on a single attribute. 
Consider a database scheme $\{Age, Gender, NativeCountry, Department, Salary\}$ %such that \begin{itemize}\item $dom(Age)=\{1,\ldots,100+\}$  \item $dom(Gender)=\{Male, Female, Other\}$\item $dom(NativeCountry)=\{US,Spain,India\}$ \item $dom(Department)=\{A/C \& Finance, R\&D, Production,$\\$ Marketing,$ $HRM, Purchasing \}$ \item $dom(Salary)=\{100K,150K,...,500K\}$ \end{itemize} 
\begin{exmp}
\textit{Query: } Count the number of records satisfying $Age \in [50,60]$\\
\textbf{Crypt$\epsilon$ Program:}
Let $\phi=(Age=50 \vee Age=51 \vee ... \vee Age=60)$ \end{exmp} $\lap_{\epsilon,1}(\countagg(\filter_{\phi}(\project_{Age}(\encD))))$
%\begin{enumerate} \item $\mathbf{\tilde{T}}_1$=\textsf{Project}($\boldsymbol{\tilde{\mathcal{D}}}$, $Age$)  \item  $\mathbf{T_2}$ = \textsf{Filter}($\mathbf{\tilde{T}}_1,\phi$)\item $\mathbf{C}$ = \textsf{Count}($\mathbf{T_2}$) \item $\hat{C}$=\textsf{Laplace}($\mathbf{C},\epsilon)$\end{enumerate}
\begin{exmp}\textit{Query: } Return the 5 most frequent age values.\\\textbf{Crypt$\epsilon$ Program:}\end{exmp}
$\noisymax^5_{\epsilon,1}(\groupbystar_{Age}(\encD))$%\begin{enumerate} \item $\mathbf{C}$=\textsf{GroupBy*}($\boldsymbol{\tilde{\mathcal{D}}},Age$)   \item $\tilde{C}$=\textsf{NoisyMax}($\mathbf{C},5,\epsilon)$\end{enumerate}
\begin{exmp}\textit{Query: } Return the marginal over attributes Age and Gender values.\\\textbf{Crypt$\epsilon$ Program:}\end{exmp}
$\lap_{\epsilon,1}(\groupbystar_{Age\times Gender}(\project_{Age \times Gender}(\crossproduct_{Age,Gender}(\encD))))$%\begin{enumerate} \item $\tilde{\mathbf{T_1}}$=\textsf{CrossProduct}$(\boldsymbol{\tilde{\mathcal{D}}},Age,Gender)$ \item $\tilde{\mathbf{T_2}}$=\textsf{Project}$(\tilde{\mathbf{T_1}}, Age \times Gender)$\item  $\mathbf{C}$=\textsf{GroupBy*}($\tilde{\mathbf{T_2}},Age \times Gender $)   \item $\hat{C}$=\textsf{Laplace}($\mathbf{C},\epsilon)$\end{enumerate}

\paragraph{\textbf{LabHE Multiplication Interaction Programs}}
Recall that labeled homomorphic encryption allows multiplication of two ciphers. Generalization to a $n$-multiplicand, $n > 2$ case can be done according to the protocol described in section \ref{genlab}. However it requires intermediate interactions with the \textsf{CSP}. Thus all Crypt$\epsilon$ programs that require multiplication of more than two ciphers need interaction with the \textsf{CSP}. 
All programs with more than three attributes in its boolean predicate would thus fall under this class.
\begin{exmp}\textit{Query:} Return the marginal over Age and Gender where NativeCountry is Mexico. \\\textbf{Crypt$\epsilon$ Program:}\\ Let $\phi$ be the condition that $(NativeCountry==Mexico) $ \begin{multline*}\lap_{\epsilon,1}(\groupbystar_{Age\times Gender}(\filter_{\phi}(\project_{Age\times Gender, NativeCountry}\\(\crossproduct_{Age,Gender}(\encD)))))\end{multline*}\end{exmp}% \begin{enumerate}\item $\tilde{\mathbf{T_1}}$=\textsf{CrossProduct} ($\boldsymbol{\tilde{\mathcal{D}}},Age,Gender$) \item $\tilde{\mathbf{T_2}}$=\textsf{Project}$(\tilde{\mathbf{T_1}}, Age \times Gender, NativeCountry)$ \item $\mathbf{T_3}$=\textsf{Filter}($\tilde{\mathbf{T_2}},\phi$)\item $\mathbf{C}$=\textsf{GroupBy*}($\tilde{\mathbf{T_2}},Age\times Gender$)\item $\hat{C}$=\textsf{Laplace}$(\mathbf{C},\epsilon)$ \end{enumerate}
\begin{exmp} \textit{Query:} Count the number of for male employees of US having age =50. \\\textbf{Crypt$\epsilon$ Program} Assume $\phi=(Age=30 \wedge Gender=Male \wedge NativeCountry=Mexico)$ \end{exmp} $\lap_{\epsilon,1}(\countagg(\filter_{\phi}(\project_{Age,Gender,NtiveCountry}(\encD))))$
%\begin{enumerate} \item $\mathbf{\tilde{T}}_1$=\textsf{Project}($\boldsymbol{\tilde{\mathcal{D}}}$, $Age,Gender,NativeCountry$)  \item  $\mathbf{T_2}$ = \textsf{Filter}($\mathbf{\tilde{T}}_1,\phi$)\item $\mathbf{C}$ = \textsf{Count}($\mathbf{T_2}$) \item $\tilde{C}$=\textsf{Laplace}($\mathbf{C},\epsilon)$\end{enumerate}
\paragraph{\textbf{Other Interaction Programs}}
 The \textsf{GroupBy} primitive requires an intermediate interaction (see section 6) with the \textsf{CSP} (for generating the encrypted one-hot-coding). The \textsf{CountDistinct} primitive also uses a Yao's garbled circuit (see section C) and hence requires a round of interaction. This in addition to the interaction required for decrypting the noisy answer (as explained above). Thus any program with the \textsf{GroupBy} or \textsf{CountDistinct} primitive requires two rounds of interaction in the least. 
\begin{exmp}\textit{Query:} Return the number of distinct age values for the male employees in the database. \\ \textbf{Crypt$\epsilon$ Program:} \\Let  $\phi=(Gender=Male)$ be the predicate such that age counts are in $\{1,...,m\}$\end{exmp} $\lap_{\epsilon,1}(\countdistinct(\groupbystar_{Age}(\filter_{\phi}(\project_{Age \times Gender}(\encD)))))$ %\begin{enumerate}\item $\mathbf{\tilde{T}}_1$=\textsf{Project}($\boldsymbol{\tilde{\mathcal{D}}}$, $Age,Gender$) \item $\mathbf{T}_2$=\textsf{Filter}($\mathbf{\tilde{T}}_1,\phi$) \item $\mathbf{T_3}$=\textsf{GroupBy*}($\mathbf{\tilde{T}}_1,Age$)\item $\mathbf{C}$=\textsf{CountDistinct}$(\mathbf{T_3})$\item $\hat{C}$=\textsf{Laplace}($\mathbf{C},\epsilon$)\end{enumerate} 
\begin{exmp}\textit{Query: } Return the number of  age values having at least 10 records in the database. \\ \textbf{Crypt$\epsilon$ Program}:\\ Let $\phi_G$ be the predicate such that age count is in $\{10,...,m\}$. \end{exmp}
$\lap_{\epsilon,1}(\countagg(\filter_{\phi}(\groupby_{Age}(\project_{Age}(\encD)))))$
%\begin{enumerate}\item $\mathbf{\tilde{T}}_1$=\textsf{Project}($\boldsymbol{\tilde{\mathcal{D}}}$, $Age$) \item $\mathbf{\tilde{T_2}}$=\textsf{GroupBy}($\mathbf{\tilde{T}}_1,Age$)\item $\mathbf{T_3}$=\textsf{Filter}$(\mathbf{\tilde{T_2}},\phi_G)$\item $\mathbf{C}$=\textsf{Count}($\mathbf{T_3}$)\item $\hat{C}$=\textsf{Laplace}$(\mathbf{C},\epsilon,)$\end{enumerate}

==> Sec-theorem.tex <==
\section{\system Security Sketch} \label{sec:security}
In this section we provide a sketch of the security proof in the semi-honest model using the well established
simulation argument~\cite{Oded}. %We assume that the reader is familiar with standard concepts, such when two distributions are computationally indistinguishable ($\equiv_c$).
\textcolor{blue}{Let program $P$ be executed on a dataset $\mathcal{D}$
with privacy parameter $\epsilon$ and let $P^{CDP}_U(\mathcal{D},\epsilon/2)$ denote the random variable corresponding to the output of running $P$ in the \textsf{CDP} model under unbounded $\epsilon/2$-DP (data size is unknown, Defn. \ref{def:unboundedDP} in \ifpaper 
the full paper \cite{anom})% using paper 
\else 
Appendix \ref{app:background}) \fi. Now, let
$P^{CDP}(\mathcal{D},\epsilon)$ denote the random variable
corresponding to the output of running $P$ in the \textsf{CDP} model under bounded $\epsilon$-DP such that  $P^{CDP}(\mathcal{D},\epsilon)\equiv (P^{CDP}_U(\mathcal{D},\epsilon/2),|\mathcal{D}|)$. Clearly by Theorem \ref{thm:boundedDP} in \ifpaper the full paper \cite{anom}% using paper 
\else 
Appendix \ref{app:background} \fi, $P^{CDP}(\mathcal{D},\epsilon)$ ensures overall bounded $\epsilon$-DP.
} \noindent
\vspace{-2mm}
\begin{theorem}\label{thm:security}
\rm
Let protocol $\Pi$ correspond to the execution of program $P$ in \system. The
views and outputs of \textsf{AS} and \textsf{CSP} are denoted as $
View_1^{\Pi}(P,\mathcal{D},\epsilon), Output_1^{\Pi}(P,\mathcal{D},\epsilon)$ and $
View_2^{\Pi}(P,\mathcal{D},\epsilon), Output_2^{\Pi}(P,\mathcal{D},\epsilon)$ respectively.
There exists Probabilistic Polynomial Time (PPT) simulators $Sim_1$
and $Sim_2$ such that:
\squishlist
\item $Sim_1 (P^{CDP}(\mathcal{D},\epsilon))$ is computationally indistinguishable ($\equiv_c$)
from $(View_1^{\Pi}(P,\mathcal{D},\epsilon),Output^{\Pi}(P,\mathcal{D},\epsilon))$, and
\item $Sim_2 (P^{CDP}(\mathcal{D},\epsilon))$ is $\equiv_c$ to
  $(View_2^{\Pi}(P,\mathcal{D},\epsilon),Output^{\Pi}(P,\mathcal{D},\epsilon))$.
  \squishend $Output^{\Pi}(P,\mathcal{D},\epsilon))$ is the combined
  output of the two parties\footnote{Note that the simulators are
    passed a random variable $P^{CDP}(\mathcal{D},\epsilon))$, i.e., the simulator is given the ability to sample
    from this distribution.}.
\end{theorem}
We detail the proof in \ifpaper 
the full paper \cite{anom}  % using paper 
\else 
Appendix \ref{sec:proof} \fi and present a brief outline here. \textcolor{blue}{In \system, measurement operators $\textsf{Laplace}$ and $\textsf{NoisyMax}$ satisfy unbounded $\epsilon/2$-DP guarantee  (noise is added from the distribution $Lap(2\cdot \Delta/\epsilon)$ in Section 5.2). Thus any \system program expressed as a sequence of transformation operators, $\bar{\mathcal{T}}$ followed by a measurement operator satisfies unbounded $\epsilon/2$-DP (Section 5.2). However, since the \AS has access to the encrypted dataset $\encD$, the dataset size is leaked. Hence the overall privacy guarantee of the whole program $P$ is bounded $\epsilon$-DP (from Theorem \ref{thm:boundedDP} in \ifpaper  full paper \cite{anom}% using paper 
\else 
Appendix \ref{app:background}) \fi.}  %Note that in \system we get only half of the $\epsilon$-DP guarantee as that of \CDP. It is so because although all the operators individually guarantee $\epsilon - $ unbounded DP, since the dataset size is revealed to the \AS, the overall privacy guarantee is that of bounded DP. Additionally, any algorithm that satisfies $\epsilon$-unbounded DP also satisfies $2\epsilon$ - bounded DP. 
One of the main
ingredients for the formal proof is the composition theorem~\cite{Oded}, which informally states: suppose a protocol $\Pi_f^g$
implements functionality $f$ and uses function $g$ as an oracle (i.e.,
uses only input-output behavior of $g$).  Assume that protocol $\Pi_g$ implements $g$ and calls to $g$ in $\Pi_f^g$ are replaced
by instances of $\Pi_g$ (we refer to this as the composite
protocol). If $\Pi_f$ and $\Pi_g$ are correct (satisfy the aforementioned simulator
definition), then the composite protocol is
correct. Thus the proof can be done in a modular
fashion as long as the underlying operators are
used in a blackbox manner (i.e. only the input-out behavior are used
and none of the internal state or messages are used).
Since every program $P$
expressible using \system operators satisfies differential privacy,
it follows from Theorem~\ref{thm:security} that every execution of
\system satisfies computational DP.
 \noindent
\begin{corollary} \vspace{-1mm}
	Protocol $\Pi$ satisfies computational differential privacy under the \textsf{SIM-CDP} notion \cite{CDP}.
\end{corollary}



Next we discuss direct extensions to the theorem.  The statement in Theorem \ref{thm:security} assumes that \textsf{AS} and \textsf{CSP} do
not collude with the users (data owners). However, if \textsf{AS}
colludes with a subset of the users $U$ , which essentially means $Sim_1$
($Sim_2$) has to be given the data corresponding to users in $U$ as
additional parameters. This presents no complications in the proof at
all (see the proof in~\cite{LReg}). If a new user $u$ joins, their
data can be encrypted and simply added to the database. We discuss how to extend the current implementation of \system to the malicious model in Section \ref{sec:malicious}. %Notice that because of the semantic-security property of the encryption scheme encryption of $d$ provides no information about encryptions of other data items. 


==> Security.tex <==
\subsection{Security Proof}\label{app:securityproof}
\eat{The involved parties in Crypt$\epsilon$ are m data owners $DO_1,\ldots, DO_m$ and two servers \textsf{AS} and the \textsf{CSP}. In this paper we consider a
semi-honest adversary  $Adv$ who can corrupt any subset of the data owners and at most one of the two
servers. This captures our assumption that the two servers are non-colluding, i.e. if one is controlled
by the adversary, the second one behaves honestly. Thus the requisite security definition should state that $Adv$ only learns the data of the corrupted data owners and the final differentially private output but nothing else about the honest data owners. In other words, the view of the adversary $Adv$ should be computationally indistinguishable from a truly differentially private protocol.
%The target ideal functionality $\mathcal{F}$ for our protocols is described in Figure \ref{ideal}. 
Answering a query in Crypt$\epsilon$ can be considered to be a two-phase protocol. In the first phase the data owners submit there data encrypted under a labeled homomorphic encryption scheme to the \textsf{AS}. Let this phase be represented by protocol $\Pi_1$. This is followed by the actual computation of the query answer via a joint computation of an equivalent Crypt$\epsilon$ program by the As and the \textsf{CSP}.  Let protocol $\Pi_2$ represent this second phase. Using this the ideal functionality of Crypt$\epsilon$ can be represented by Figure \ref{ideal}. 
 \eat{\begin{figure}\noindent
\framebox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{\itshape \textbf{Parties}:- \textsf{AS}, \textsf{CSP} and $\textsf{DO}_i$, $\forall i \in \{1,...,m\} \\ \textbf{Input}:-  D_i, \forall i \in \{1,...,m\} , \thinspace\thinspace\thinspace\thinspace\thinspace\thinspace\textit{Query Q}, \textit{Privacy Parameter } \epsilon$ \\
\textbf{Output}:- $\epsilon-$Differentially private output for Q, $\hat{c}$\\\\\textbf{Phase 1:} \textsf{AS}, \textsf{CSP} and $\textsf{DO}_i$ jointly run protocol $\Pi_1$\\\textbf{Phase 2:} \textsf{AS} and \textsf{CSP} run protocol $\Pi_2$ to generate $\hat{c}$ }}  \caption{Ideal functionality $\mathcal{F}$ of Crypt$\epsilon$} \label{ideal} \end{figure}}
To formally prove the security, we use the standard simulation based definition \cite{Goldreich}.
Let us consider a public function $\phi: (\{0,1\}^k)^n\mapsto \{0,1\}^t$ and let $P_1; \cdots ; P_n$ be $n$ players modeled
as PPT machines. Each player $P_i$ holds the value $x_i \in \{0,1\}^k$ and wants to compute the
value $\phi(x_1;\cdots ; x_n)$ while keeping his input private. The players can communicate among
them using point-to-point secure channels in the synchronous model. If necessary, we
also allow the players to use a broadcast channel. To achieve their goal, the players jointly
run a $n$-party MPC protocol . The latter is a protocol for $n$ players that is specified via the
next-message functions: there are several rounds of communication and in each round the player $P_i$ sends to other players a message that is computed as a deterministic function
of the internal state of $P_i$ (his initial input $x_i$ and his random tape $k_i$) and the messages
that $P_i$ has received in the previous rounds of communications. The view of the player $P_j$
,
denoted by $ViewP_j()$
(a1, . . . , an), is defined as the concatenation of the private input aj
, the
random tape kj and all the messages received by Pj during the execution of $\Pi$. Finally, the
output of $\Pi$ for the player $P_j$ can be computed from the view ViewPj
. In order to be private,
the protocol $\Pi$ needs to be designed in such a way that a curious player $P_i$ cannot infer
information about $x_j, j \neq i$  from his view $ViewP_i$.
More precisely, we have the following definition.

\begin{definition}  Let $S$ a subset of at most $n - 1$ players, the protocol $\Pi$ realizes $\phi$ with privacy against
$S$ if it is correct and there exists a PPT algorithm $Sim$ such that $(ViewP_i)_{P_i\in S}$ and
$Sim(\{x_i,P_i\in S\} , \phi(x_1, . . . , x_n))$ are computationally indistinguishable for all inputs.
 \end{definition}
%Let us list the interactions of the cSP - the \textsf{CSP} has no interactions with the data owners ever. Moreover which prevents the . Always decrypt the nout is always a . Hence it 
%From the For the it can thus $\delta$ comes from the  Next
The evaluation of any Crypt$\epsilon$ program can  be seen as an MPC for m + 2 parties: $\textsf{DO}_1, . . . , \textsf{DO}_m$, \textsf{AS} and
\textsf{CSP}.

\begin{theorem}Let $S \subset \{1,...,m\}$ then $\Pi$ realizes $\psi$  with correctness and privacy against
the adversaries $Adv_1=\textsf{AS} \cup \{\textsf{DO}_i, i \in S\}$  and $Adv_2=\textsf{CSP} \cup  \{ \textsf{DO}_i, i \in S\} $\end{theorem}}
\begin{proof} \begin{comment}The interactions between the \textsf{AS} and the \textsf{CSP} can be categorized into three types \begin{enumerate}\item Yao's garbled circuits - Primitives: NoisyMax, CountDistinct\item Decryption of masked data - Primitives: GroupBy \item Decryption of differentially private output- Primitives: Laplace \end{enumerate} Thus there are three possibilities for protocol $\pi_2$. For the garbled circuit based protocol $\pi_2$, the output of both the primitives NoisyMax and CountDistinct are differentially private by definition.  Hence by the standard semantic security of garbled circuits \cite{Yao, yao2}, the protocol is secure against a P.P.T adversary revealing nothing other than the differentially private  circuit outputs. 
We will discuss the simulators for the other two cases as follows starting of with the second case, i.e., when the \textsf{CSP} decrypts masked data.
\end{comment}
Let simulators $Sim_1$ and $Sim_2$ simulate the view of ${Adv}_1$ and $Adv_2$ respectively. 
From our discussion in the following primitives result in an interaction between the \textsf{AS} and the \textsf{CSP}.
\squishlistnum \item \textsf{GroupByCount} \item \textsf{CountDistinct} \item  \textsf{NoisyMax} \item {Laplace} \squishendnum 
Out of these four, primitives \textsf{GroupByCount} and \textsf{CountDistinct} are implemented via garbled circuits with differentially private outputs. Thus these are secure by the semantic security of garbled circuits and their proof is not presented here.
We present the proof for the other two interactions here. First let us look at the interaction for the \textsf{GroupByCount} primitive. Let $l$ be the length of the data-records when expressed in the suitable attribute-wise one-hot-coding representation and let $\tilde{\mathcal{V}}$ denote the output from \textsf{CSP}.  
$\mathcal{S}_1=Sim_1(\{D_i, i \in S\}, labEnc_{pk}(\tilde{\mathcal{V}}), pk)$
\begin{enumerate}\item Run $Gen(\kappa)\mapsto (pk,sk)$ 
\item Draw $M \in_R [m]^{s_A}$
\item Compute $\mathbf{\tilde{V}}'[i]=RightRotate(\mathbf{\tilde{V}},M[i]), i \in [s_A]$
\item For all $i \in \{1,...,m\}$ if $i \in S$ then encrypt $D_i$. 
Otherwise compute $labEnc_pk(D_i)$ as a random $l$-lengthed vector $r_i \in \mathcal{C}^l$. [We abuse the notation slightly here, $labEnc_pk(D_i)$ denotes component wise encryption of the record represented in per-attribute one-hot-coding]
\item Output $\Big(\{D_i, i \in S\},pk,D',\mathbf{\tilde{V}}' \Big)$ where $D'=\{r_i\},i \in \{1,...,m\} i \not \in S$ as computed in step 4.
\end{enumerate}
It follows from the semantic security of the encryption scheme that the simulation
output has the same distribution as that of the views of the corrupted parties in $Adv_1$.\\
$\mathcal{S}_2=Sim_2(D_i, i \in S)$
\begin{enumerate}\item Run $Gen(\kappa)\mapsto (pk,sk)$ \item Sample $\mathcal{R} \in_R [m]^{s_A}$
\item Convert $\mathcal{R}$ to its one-hot-coding representation $\tilde{\mathcal{R}}$
\item Output $\Big(\{D_i, i \in S\},labEnc_{pk}(\tilde{\mathcal{R}}) \Big)$
\end{enumerate}
Thus the simulation output has the same distribution of the
views of the corrupted parties in $Adv_2$. 

  Note that a sequence of transformations followed by a \textsf{Laplace} primitive is a valid \system program that should satisfy $\mathcal{F}$. We capture this in our discussion below. Recall that in \system for the \textsf{Laplace} primitive both the \textsf{AS} and the \textsf{CSP} adds separate instances of Laplace noise to the output. Let the noise added by the \textsf{AS}  be denoted as $\eta_1$ and the one added by the \textsf{CSP} be denoted as $\eta_2$\\
$\mathcal{S}_1=Sim_1(\{D_i, i \in S\}, \hat{c}, \eta_1)$
\begin{enumerate}\item Run $Gen(\kappa)\mapsto (pk,sk)$ 
\item Draw $\eta_1 \in Lap(\frac{1}{\epsilon})$
\item Compute $c'=\hat{c}-\eta'-\eta_1$
\item For all $i \in \{1,...,m\}$ if $i \in S$ then encrypt $D_i$. 
Otherwise compute $labEnc_pk(D_i)$ as a random $l$-lengthed vector $r_i \in \mathcal{C}^l$. [We abuse the notation slightly here, $labEnc_pk(D_i)$ denotes component wise encryption of the record represented in per-attribute one-hot-coding]
\item Output $\Big(\{D_i, i \in S\},D',labEnc_{pk}(c'),c+\eta'+\eta_1 \Big)$ where $D'=\{r_i\},i \in \{1,...,m\} i \not \in S$ as computed in step 4.
\end{enumerate}
It follows from the semantic security of the encryption scheme that the simulation
output has the same distribution as that of the views of the corrupted parties in $Adv_1$ in the
protocol $\pi$.\\
$\mathcal{S}_2=Sim_2(D_i, i \in S, \hat{c}=c+\eta_1+\eta_2)$
\begin{enumerate}\item Run $Gen(\kappa)\mapsto (pk,sk)$ \item $\bar{c}=\hat{c}-\eta_2=c+\eta_1$
\item Output $\Big(\{D_i, i \in S\},labEnc_{pk}(\bar{c}),\hat{c} \Big)$
\end{enumerate}
Thus the simulation output has the same distribution of the
views of the corrupted parties in $Adv_2$ in the protocol $\Pi$. 


\end{proof}
\eat{\begin{table}[h!]
\small
\centering
\caption {Comparative analysis of the different DP models}
\scalebox{0.7}{ \begin{tabular}{|l| c c c|}  \toprule
\multicolumn{1}{|c}{\textbf{Features}} & \textbf{LDP}  & \textbf{CDP}  & \textbf{Crypt$\epsilon$}  \\ [0.5ex] 
 \hline \hline\# Servers & 1& 1 & 2\\\hline
Trust  & & & Untrusted \\  Assumption & Untrusted & Trusted & Semi Honest \\for Server &  &   &  Non-Colluding  \\ \hline
Data Storage & \multirow{2}{*}{Noisy} & \multirow{2}{*}{Clear} & \multirow{2}{*}{Encrypted} \\in Server & &  &  \\\hline
Adversary & Unbounded & Unbounded & Bounded \\\hline
 Error & $O\Big(\frac{\sqrt(n)}{\epsilon}\Big)$& $O\Big(\frac{1}{\epsilon}\Big)$ & $O\Big(\frac{1}{\epsilon}\Big)$\\\hline
 Impossibility & Everything & Algorithms w/ & Same as that \\results & beyond SQ model & Unbounded Sensitivity & of \textsf{CDP}\footnotemark\\
  [1ex] 
 \bottomrule
 \end{tabular}}\label{DPCompare}
\end{table}
\footnotetext{Theoretically no restriction, however practical constraints maybe present}}


==> discussion.tex <==
\section{Discussion}
\subsection{Joint Laplace Noise Generation}\label{jointLap}
Recall that in \system,  both the servers, \textsf{AS} and \textsf{CSP} have to add two separate instances of Laplace noise to true answer. Thus the expected error incurred in \system is quantitatively twice that of the traditional Laplace mechanism in traditional \textsf{CDP} model. However, there is an alternative way of jointly computing a single instance of the Laplace noise via a secure multi party computation protocol~\cite{Djoin}. For this, the \CPS generates a garbled circuit that takes one $l$-bit random string from \CPS and \AS each as an input, denoted by $S_1$ and $S_2$ respectively. This circuit performs$S=S_1 xor S_2$  and uses it to generate an instance of random noise, $\eta$ drawn from the distribution $Lap(\frac{1}{\epsilon})$ following the fundamental law of transformation of probabilities.
Last, the circuit encrypts $\eta$ and returns $\boldsymbol{\eta}=labEnc_{pk}(\eta)$.
Hence, this approach adds just one instance of the Laplace noise, resulting the same accuracy guarantee as the \textsf{CDP} model. However owing to the garbled circuit, this implementation is computationally heavier. Therefore, we choose the two phase noise addition implementation for \system in this paper.

\eat{\begin{enumerate}\item takes a $l$-bit random string, $S_1$ as an input from the \textsf{CSP}
    \item takes another $l$-bit random string $S_2$ as an input from the \textsf{AS} \item performs $S=S_1 xor S_2$  and uses it to generate an instance of random noise, $\eta$ drawn from the distribution $Lap(\frac{1}{\epsilon})$ following the fundamental law of transformation of probabilities \item encrypts $\eta$ and returns $\boldsymbol{\eta}=labEnc_{pk}(\eta)$\end{enumerate}}


\subsection{Separation from LDP model}\label{app:sepldp}
As discussed in the introduction, the \textsf{LDP} model is less powerful in query answering than the \textsf{CDP} model~\cite{Kasivi,mixnets}. However, by virtue of secure computation, we can potentially implement all the functionalities of the \textsf{CDP} model in our two-server model. However, by virtue of secure computation, we can potentially implement all the functionalities of the \textsf{CDP} model in our two-server model. Functional efficiency might be a point of contention in certain cases, but nothing in the architecture of  \system can restrict its algorithmic expressibility. Recall that the power of the \textsf{LDP} model is equivalent to that of the statistical query model \cite{SQ1} from learning theory and there exists an exponential separation between the accuracy and sample complexity of local and central algorithms~\cite{Kasivi}.

We will showcase three different queries which can be computed efficiently in \system but infeasible in the standard \textsf{LDP} model.

\stitle{DNF Queries.}
The class of DNF queries fall outside the scope of statistical query models \cite{DNF}. Hence it is infeasible to answer counting queries based on a predicate with a disjunction in the \textsf{LDP} model. However, we can answer them in \system as follows.
Consider a DNF query 
$$\phi = (A_{11}\land ...\land A_{1k}) \vee ... \vee (A_{t1}\land ... A_{tl}), t, k,l \in \mathcal{Z}_{\geq 0}.$$

Let $Attribute(\phi)$ denote the set of all attributes in $\mathcal{A}$ that appear in the boolean condition $\phi$. For example, if $$\phi = \big((\mathcal{A}_1==v_1) \land \mathcal{A}_2==v_2) \vee \mathcal{A}_3==v_3 \big),$$ then we have $Attribute(\phi)=\{\mathcal{A}_1, \mathcal{A}_2,\mathcal{A}_3\}$.

Firstly, the \AS computes the attribute set $\bar{A}=Attribute(\phi)$ and projects $\encD$ on $\bar{A}$. Then, the \AS constructs the encrypted one-hot-coding of over all attributes in $\bar{A}$ using the cross product transformation. We denote the new attribute $A'$ and the new table $\encD'$. Now, the \AS simply filters this new table $\encD'$ with predicate $\phi'$  such that $\phi'$ is the equivalent of $\phi$ when expressed in terms of the new  attribute $A'$. Finally, \AS  performs the \textsf{Count} transformation and the \textsf{Laplace} transformation to obtain the final result.

\eat{
\begin{enumerate}\item Firstly, the \textsf{AS} computes the attribute set $A^*=Attribute(\phi)$.
\item Next the \textsf{AS} performs a \textsf{Project} transformation on inputs attribute set $A^*$ and the entire encrypted database $\boldsymbol{\tilde{\mathcal{D}}}$. 
\item Let $A^*= \{A^*_1,A^*_2,\ldots,A^*_t\}, t \leq k$. The \textsf{AS} constructs the encrypted one-hot-coding over the entire $t$-dimension $\lq$attribute' $\mathcal{A}^*=\times_{i=1}^t A^*_i$ by $(t-1)$ iterative application of the cross product transformation. 
\item Note that the result of the preceding step is a $m\times 1$ table where the $i^{th} , i \in [m]$ record corresponds to the encrypted one-hot-coding over the entire $t$-dimension domain space of $\mathcal{A}^*$ of data owner $\textsf{DO}_i$. Now the \textsf{AS} simply applies the \textsf{Filter} transformation on this table with predicate $\phi'$  such that $\phi'$ is the equivalent of $\phi$ when expressed in terms of the new  attribute $\mathcal{A}^*$.
\item This is followed by performing the \textsf{Count} transformation and the \textsf{Laplace} transformation to obtain the final result. 
\end{enumerate}
}

\stitle{Variable Selection Problem.} The variable selection problem is an optimization problem described as follows. Given a set of counting queries, the problem finds the query with nearly the largest value, i.e., computes an approximate argmax. Cheu et al.~\cite{mixnets} prove that the sample complexity of this problem in the "one-message" mixnet model (i.e., each user send only a single message into the shuffle) is exponentially larger than that of the \textsf{CDP} model. The variable-selection problem is actually equivalent to the exponential mechanism~\cite{Dork} in the \textsf{CDP} model. Moreover, the exponential mechanism is simply a variant of the "Report Noisy-Max" algorithm with a different noise distribution \cite{Nm}.  Thus essentially, the \textsf{NoisyMax} primitive in \system is capable of solving the variable-selection problem accurately.

\stitle{Count Distinct Values.} Consider the problem of computing the number of distinct values out of a set of $m$ user data where the domain of the values is $S$ and $m<<|S|$. In the \textsf{LDP} model, for small sizes of $S$, one can construct a frequency oracle and compute the number of values with non-zero count with some careful thresholding~\cite{LDP1}. However, if the size of $S$ is huge then it becomes computationally infeasible to deploy the aforementioned mechanism. For example, if the values correspond to different URLs, since the total domain size is $2^{64}$, computation limitations make this problem infeasible to be solved in the \textsf{LDP} setting. There are mechanisms that use techniques like dividing the data into groups and then performing specialised processing etc to find top k heavy hitters in this setting \cite{HH,HH2} but still these work only for low values of $k<60$.  Although for our discussion in the paper we have considered the one-hot-coding as our preferred data encoding scheme, \system architecturally can support any arbitrary encoding scheme.  For instance, for URLs the data owners can instead use the domain name based encoding (i.e., subdomain.secondleveldomain.topleveldomain) for encrypting their data. Following this, an appropriate garbled circuit to count the number of distinct values from this encrypted dataset (which can be defined as a new Crypt$\epsilon$ primitive) can answer the above query in the \system setting.

\begin{comment}\subsection{Answering queries with disjunctions in predicate} Now let us consider a DNF query predicate $\phi=\phi_1 \vee \phi_2$ where $\phi_1=(A_1==v_1 \wedge \ldots \wedge A_n==v_n)$ and $\phi_2=(A'_1==v'_1 \wedge \ldots \wedge A'_n==v'_n)$ are two conjunctive clauses. For a given record assume, \begin{gather*}\mathbf{d}=\mathbf{c_1}\oplus \mathbf{c_2}-labMult(\mathbf{c_1,c_2}) \\
\mathbf{c_1}=genLabMult(\mathbf{\tilde{R}}_{A1}[v_1], \ldots ,\mathbf{\tilde{R}}_{An}[v_n] ) \\ \mathbf{c_1}=genLabMult(\mathbf{\tilde{R}}_{A1}[v_1], \ldots ,\mathbf{\tilde{R}}_{An}[v_n] )\end{gather*} Note that $d=1$  only iff  the record satisfies $\phi$. Thus for a two clause  DNF predicate as above, the optimized Filter transformation takes as input $x \times y$ encrypted table $\tilde{\mathbf{T}}$ with attribute set $\bigcup_{i=1}^n Attribute(\phi_i)$ and outputs a $x \times 1$ encrypted table $\mathbf{\tilde{T}}'$ such that \begin{gather} \mathbf{\tilde{T}}'[i]= \mathbf{c_1}\oplus \mathbf{c_2}-labMult(\mathbf{c_1,c_2}) \\
\mathbf{c_1}=genLabMult(\mathbf{\tilde{R}}_{A1}[v_1], \ldots ,\mathbf{\tilde{R}}_{An}[v_n] ) \\ \mathbf{c_1}=genLabMult(\mathbf{\tilde{R}}_{A1}[v_1], \ldots ,\mathbf{\tilde{R}}_{An}[v_n] )\end{gather} For $t>2$ clauses in a DNF, apply the Filter transformation pairwise for $\lceil \log t \rceil$ iterations. 
\end{comment}

An important point to be noted here is that the power of the shuffler or mixnet model  (which is obtained by augmenting \textsf{LDP} with anonymization via shuffling)~\cite{Prochlo, mixnets,amplification},  lies strictly between that of traditional \textsf{LDP} and \textsf{CDP}. Thus the two-server model of Crypt$\epsilon$ differs from this line of work in three major ways. First, \system results in no reduction in expressibility as compared to that of the \textsf{CDP} model. Second, the mixnet/shuffler model results in an approximate DP guarantee $(\epsilon\sqrt{\frac{\log\frac{1}{\delta}}{n}},\delta)$ which incurs an expected error of $O(\epsilon\sqrt{\log\frac{1}{\delta}})$.  In practice, $\delta$ has to be smaller than $\frac{1}{n}$ in order to get  meaningful privacy. In contrast, \system achieves the same order of accuracy guarantees as that of the \textsf{CDP} model. Finally, the trust assumptions of the shuffler/mixnet model differ from that of \system. Google's implementation relies on a trusted intermediary shuffler which they implement via trusted hardware enclaves. However truly secure hardware enclaves are notoriously difficult to achieve in practice \cite{Foreshadow}. The mixnet model on the other hand requires a  mix network or mixnet which is a protocol involving several computers that inputs a sequence of encrypted messages, and outputs a uniformly random permutation of those messages' plaintexts.  Their trust assumption is that at least one of the servers needs to behave honestly. For \system, both the servers are completely untrusted under the constraint that they are non-colluding and follow the protocols semi-honestly.


==> system_description.tex <==

\begin{table}[t]
\centering
\caption {Notations}
\scalebox{0.7}{
 \begin{tabular}{l|l}  \toprule
 \multicolumn{1}{c}{\textbf{Symbol} } &  \multicolumn{1}{c}{\textbf{Explanations}}\\\midrule
\textbf{Boldface}& \text{- represents encrypted data}\\
$\tilde{}$ & \text{- represents one-hot-coding}  \\  $\hat{}$ & - represents a differentially private output  \\ $A$ &- an attribute  \\ $s_A$ &- size of domain of attribute $A$
\\$dom(A)=\{v_1,\ldots,v_{s_A}\}$ & - domain of attribute $A$\\ $ct_{A,i}$  &- \# \text{records with value $v_i$ for attribute} A\\ $m$   &- \text{\# number of data onwers}\\ $\boldsymbol{\tilde{\mathcal{D}}}$  &- \text{encrypted database with records in}\\&\text{  per-attribute one-hot-coding } \\ %$\mathcal{A}=\{\mathcal{A}_1,...\mathcal{A}_l\}$   &- \text{set of attributes in the schema of $\boldsymbol{\tilde{\mathcal{D}}}$}\\
$x \times y \text{ table } \mathbf{T}$   &- \text{an encrypted table  with $x$ records in}\\&\text{ one-hot-coding and $y$ columns one for}\\&\text{ each attribute; serves as one of the }\\&\text{ inputs to a transformation primitive}\\ $\mathbf{B}$&- \text{a vector of length $m$ such that each entry}\\&\text{ $\textbf{B}[i]$ represents whether record $r_i, i \in [m]$}\\& \text{is relevant to the program at hand} \\ $V$ & -\text{ represents a vector}\\$c$ &- \text{represents a scalar}\\$\mathcal{P}$ & - \text{represents a set}\\
 \bottomrule
 \end{tabular}}
 \label{Notations}
\end{table}

%$Attribute(\phi)$ - The set of attributes that appear in the boolean condition $\phi$\\
%$\mathcal{I}(A)$- Denotes the integral representation of $dom(A)$\\$\mathcal{I}_A(\phi)$- Denotes the elements in $\mathcal{A}$ that satisfies $\phi$

\section{System Overview}\label{sec:overview}

\begin{figure}
<<<<<<< HEAD
\includegraphics[width=\columnwidth]{diag.png}\caption{ Crypt$\epsilon$ System Setting: The  \textsf{AS} runs the Crypt$\epsilon$ programs. The \textsf{CSP} manages the cryptographic primitves. } \end{figure}
%This section provides an overview of \system. We begin this section with the desiderata for \system that motivates our design followed by a discourse on the different components of \system and their functionality. Next we discuss about a few additional architectural choices we make for \system. This is followed by a description of \system's trust model and security sketch.
=======
\includegraphics[width=\columnwidth]{diag.pdf}\caption{ Crypt$\epsilon$ System Setting: The  \textsf{AS} runs the Crypt$\epsilon$ programs. The \textsf{CSP} manages the cryptographic primitves. } \end{figure}
This section provides an overview of \system. We begin this section with the desiderata for \system that motivates our design followed by a discourse on the different components of \system and their functionality. Next we discuss about a few additional architectural choices we make for \system. This is followed by a description of \system's trust model and security sketch.
>>>>>>> 176d67e3738bd609e2fcc15154a196b98aa6fc77

In this section, we describe \system's architecture (Sec~\ref{sec:arch}), the different modules in the system (Sec~\ref{sec:modules}), and the trust assumptions made by our system (Sec~\ref{sec:trust}). We end with a brief discussion justifying the design of \system (Sec~\ref{sec:discuss-arch}). 

\eat{\subsection{Crypt$\epsilon$ Design}
The  desiderata for  the functionality of \system are as follows
\squishlist \item The architecture of \system should be able to support any differentially private algorithm that is permitted in the \textsf{CDP} model at the same order of accuracy guarantee as that of \textsf{CDP}, i.e. constant $O(\frac{1}{\epsilon})$ error bound.
\item Raw data records cannot be stored in the clear in any server, i.e., the server(s) in \system are untrusted. 
\item Data owners must be  off-line.\squishend
Recall from our discussion in section 1, \textsf{CDP} gives constant error bounds, however it relies on a trusted server for this. In contrast \textsf{LDP} requires no trusted server but results in limited accuracy.  The first two principles thus capture \system's objective of achieving the "best of both worlds", i.e., the accuracy guarantees and expressibility of the \textsf{CDP} model with  trust assumptions similar to that of the \textsf{LDP} model. The third principle stems from the fact that another undesirable trait of \textsf{LDP} is its inherent requirement for the data owners to be on-line during every query processing.  This is so because  in \textsf{LDP} %the private data of the individuals are not collated at a single place and hence%
depending on the query at hand, every time the data owners need to compute a different noisy measurement that best answers it. This is in general a poor practice as maintaining active communication channels for all the data owners might be unwieldy. \par The first desideratum can be achieved if we collate the data into a single data set such that any measurement can be performed on the entire data set at once followed by a single  instance of noise addition as opposed to aggregation over noisy measurements on individual data. The second desideratum mandates that the data hence collected should be suitably protected via cryptographic primitives (e.g. encryption scheme). Thus the first two requirements combined, necessitates \system to be able to perform differentially private computations on the encrypted data itself. This leads us to use linear homomorphic encryption and secure computation (specifically Yao's garbled circuits)  as the cryptographic primitives of our choice for \system. Note, by virtue of secure computation, we can potentially implement all the functionalities of the \textsf{CDP} model in \system. However, bearing the practical efficiency of the cryptographic primitives in mind, we impose certain limitations on the expressibility of \system. Due to the third desideratum, a generic $m+1$ party secure computation is ill-suited for our setting. This requires a third party entity that can factor out the onus of participating in a secure computation protocol from the data owners and capture its functionality in (at least) a 2-party protocol instead.   Moreover, since the data owners are no longer in the loop to monitor every query answering, the aforementioned entity should also watchdog the overall privacy budget expenditure. 
Guided by the above principles we design a two-server model for \system with the following components
\\(1)\textbf{ Data-Owners (\textsf{DO})} -  Each data-owner $\textsf{DO}_i, i \in [m]$ has  a
private data record $D_i$ and is willing to share it only if encrypted.   \\(2)\textbf{ Analytics Server (\textsf{AS})} - The \textsf{AS} wants to run a set of differentially private programs on the dataset $\mathcal{D}=\bigcup_{i=1}^m D_i$  but has 
access only to the encrypted copies of $D_i, i \in [m]$.
\\(3)\textbf{ Cryptographic Service Provider (\textsf{CSP})} -
 The \textsf{CSP} manages the cryptographic primitives used in Crypt$\epsilon$ and interacts with the \textsf{AS} to compute the
noisy answers. It is also responsible for monitoring the overall privacy budget expenditure.
%\xh{Rather than providing all the encryption details, can we just simply have an algorithm box to summarize the interactions between these three components. Then describe the interactions and highlight the key functionalities of each component, and then the trust model. }
}

\subsection{System Architecture}\label{sec:arch}

 
 
\subsection{\system Modules}\label{sec:modules}

\stitle{Cryptographic Service Provider (\textsf{CSP})}\\
(1)\textbf{ Key Manager }- The foremost duty of the \textsf{CSP} is to initialize the encryption scheme of Crypt$\epsilon$. This task is handled by the \textit{Key Manager} module which generates the key pair $(sk,pk)$ for the \textsf{labHE} scheme. It stores the secret key, $sk$ with itself and releases the public key, $pk$. Note that since the \textsf{CSP} has exclusive access to the secret key $sk$, it is the only entity capable of decryption in Crypt$\epsilon$.\\
(2)\textbf{ Data Decryption }- The \textsf{CSP} being the only entity capable of decryption,  any measurement of the data (even noisy) has to involve the \textsf{CSP}. The \textit{Data Decryption} module is tasked with handling all such interactions with the \textsf{AS}. \\
(3)\textbf{ Privacy Engine }- Crypt$\epsilon$ starts of with a total privacy budget of $\epsilon^B$ which is unanimously agreed upon by all the data owners. Note that the mechanism of deciding $\epsilon^B$ should be piloted by social prerogatives \cite{e1,e2} 
and is currently outside the scope of Crypt$\epsilon$. For executing any program, the \textsf{AS} has to interact with the \textsf{CSP} at least once (for decrypting the noisy answer) thereby giving the \textsf{CSP} the opportunity to monitor the \textsf{AS}'s actions in terms of privacy budget expenditure. The \textit{Privacy Engine} module hence maintains a public ledger that records the privacy budget spent in executing each program. Once the privacy cost incurred reaches 
$\epsilon^B$, the \textsf{CSP} refuses to decrypt any further answers thereby ensuring that the privacy budget is not exceeded.  The ledger is completely public allowing any data owner to verify it as and when desired.\\
\stitle{Data Owners (\textsf{DO})}\\
(1)\textbf{ Data Encoder} -  Each data owner $\textsf{DO}_i, i \in [m]$ has a private data record $D_i$ of the form $\langle A_1,...A_l\rangle$ where ${A}_j$ is an attribute. At the very outset, every data owner  $\textsf{DO}_i$ represents his/her private record $D_i$ in its respective per attribute one-hot-coding format. The one-hot-coding is a way of representation for categorical attributes and is illustrated by the following example. 
If the database schema in \system is given by  $\langle Age,Gender\rangle$ then corresponding one-hot-coding representation for a data owner $DO_i, i \in [m]$ with the record $\langle 30, Male\rangle$, is given by $\tilde{D_i}=\langle[\underbrace{0,\ldots,0}_{29},1,\underbrace{0,\ldots,0}_{70}],[1,0]\rangle$. \\
(2)\textbf{ Data Encryption} - The \textit{Data Encryption} module stores the public key $pk$ of the labHE scheme used in Crypt$\epsilon$ which is announced by the CSP. This key is used for an element-wise encryption of the data owner's  record of per attribute one-hot-codings. In our aforementioned example, we get $\mathbf{\tilde{D}}=\langle[\underbrace{labEnc_{pk}(0),\ldots}_{29},labEnc_{pk}(1),\\\underbrace{\ldots,labEnc_{pk}(0)}_{70}],
[labEnc_{pk}(1),labEnc_{pk}(0)]\rangle$. Finally the data owner sends this encrypted record to the \textsf{AS} via a secure channel. This is the only interaction that a data owner ever participates in, all the program executions are carried out by the \textsf{AS} and the \textsf{CSP} with the data owners being completely off line.\\
\stitle{Analytics Server (\textsf{AS)}}\\
(1)\textbf{  Aggregator} - The \textit{Aggregator} collects the encrypted records $\mathbf{\tilde{D_i}}$ from each of the data owners $\textsf{DO}_i$ and collates them into a single encrypted database $\boldsymbol{\tilde{\mathcal{D}}}$. %Note that in contrast, the server in the \textsf{CDP} model, being trusted, stores the data in the clear whereas in the \textsf{LDP} model the untrusted server stores appropriately randomized (noisy) data.   
\\(2)\textbf{ Program Executor }- The \textit{Program Executor} is the most important module of the \textsf{AS} and is tasked with the execution of Crypt$\epsilon$ programs. It takes as input a Crypt$\epsilon$ program from an external data analyst, alongside the appropriate privacy parameter $\epsilon$ and publishes the differentially private output computed with the assistance of the \textsf{CSP}. Crypt$\epsilon$ supports a set of 9 primitives and a Crypt$\epsilon$ program is an execution plan expressed as a sequence of these primitives. The primitives can be broadly classified into two types- transformation primitives and measurement primitives. Transformation primitives allow certain modifications on the encrypted data and are performed almost entirely by the \textsf{AS}. The measurement primitives on the other hand reveal some noisy measurement of the data and requires interaction with the \textsf{CSP}. \system supports two types of measurement primitives that implement two of the most popular differentially private mechanisms, Laplace mechanism \cite{Dork} and Noisy-Max \cite{Dork}. A typical Crypt$\epsilon$ program execution consists of  a series of transformation on the encrypted data followed by a measurement primitive and arbitrary post-processing. \\
 \textit{Noise Addition in \system} - For the Laplace mechanism, both the \textsf{AS} and the \textsf{CSP} add two separate instances of the random noise to the program output. This is necessary because had only one of them added the noise, then after the release of the clear text output, that party can simply subtract out the noise to reveal the true private answer. An alternative way can be both \AS and \CSP jointly computing a single instance of the noise using a secure computation protocol (see Appendix D.1). However, we do not implement it in the current version of \system as the two-fold noise addition is more efficient. For the Noisy-Max primitive, we provide an efficient secure computation protocol where only a single instance of noise by either party suffices. 
Since in Crypt$\epsilon$ the point of noise addition is just at the two servers, unlike at every individual in \textsf{LDP}, we achieve constant error bounds which is of the same order as that of \textsf{CDP} (see section \ref{exp:results}). 
\subsection{Crypt$\epsilon$ Workflow}
The complete workflow of Crypt$\epsilon$ is outlined as follows\\(1) \textbf{ Setup Phase} - This is the very first step in Crypt$\epsilon$ where the key manager of \textsf{CSP} generates the key pair for labHE $(sk,pk)$, publishes $pk$ and stores $sk$. \\(2) \textbf{ Data Collection Phase }- In the next phase, the $\textit{Data 
Encoder}$ and $\textit{Data Encryption}$ modules of every data owner, work to produce the encrypted data records which are then submitted to the \textsf{AS}. The data owners are relieved of all other duties and can go completely off-line. The $\textit{Aggregator}$ module of the \textsf{AS} then aggregates these encrypted records into a single encrypted database $\boldsymbol{\tilde{\mathcal{D}}}$. \\(3) \textbf{ Program Execution Phase} - In this phase, the \textsf{AS} executes a Crypt$\epsilon$ program with some interaction with the \textsf{CSP}  and generates a differentially private output.  \\
The \emph{Setup} and \emph{Data Collection} phases occur just once at the very beginning, every subsequent program  is handled via the corresponding  \emph{Program Execution} phase. Figure 1 shows the diagrammatic representation of \system. A comparative analysis of \system, \textsf{CDP} and \textsf{LDP} is presented in  Table \ref{DPCompare}.
\begin{table}[h!]
\centering
\caption {Comparative analysis of the different DP models}
\scalebox{0.7}{ \begin{tabular}{|c| c c c|}  \toprule
\multicolumn{1}{|c}{\textbf{Features}} & \textbf{LDP}  & \textbf{CDP}  & \textbf{Crypt$\epsilon$}  \\ [0.5ex] 
 \hline \hline\# Centralized Servers & 1& 1 & 2\\\hline
Trust Assumption & & & Untrusted \\   for Centralized & Untrusted & Trusted & Semi Honest \\ Server &  &   &  Non-Colluding  \\ \hline
Data Storage & \multirow{2}{*}{N/A} & \multirow{2}{*}{Clear} & \multirow{2}{*}{Encrypted} \\in Server & &  &  \\\hline
\multirow{2}{*}{Adversary} & Information & Information & Computationally \\& Theoretic & Theoretic & Bounded\\\hline
 Error on Statistical Counting Query& $O\Big(\frac{\sqrt(n)}{\epsilon}\Big)$& $O\Big(\frac{1}{\epsilon}\Big)$ & $O\Big(\frac{1}{\epsilon}\Big)$\\
  [1ex] 
 \bottomrule
 \end{tabular}}\label{DPCompare}
\end{table}
%\footnotetext{For practical constraints the current implementation has restrictions}
 %in between that of the central differential privacy model and the local differential privacy model - although it is definitely much weaker than that of the central differential privacy model, Crypt$\epsilon$'s trust model is slightly stronger as compared to that of the local differential privacy model owing to the aforementioned premises. 
%The formal security analysis for \system is presented in Appendix section B. 
\begin{comment}
learn any other information about the private datasets Di beyond what is revealed by the
model itself. Even in the case that one of the two servers (MLE or CSP) colludes with some
of the data-owners, they should learn no extra information about the data held by the
honest data-owners. In order to achieve this goal we design a system that can be seen as
multi-party protocol run by the m +2 parties mentioned before and specified by a sequence
of steps. This system (described in Section 4) has the following two-phase architecture:
We assume that the Evaluator and the CSP do not
collude. Each one may try to subvert the system as
discussed above, but they do so independently. More
precisely, at most one of these two parties is malicious:
this is an inherent requirement without which security
cannot be achieved.
• We assume that the setup works correctly, that is all
users obtain the correct public key from the CSP. This
can be enforced in practice with appropriate use of
Certificate Authorities.
Note that is true for any cryptographic primitive and is 
The can actually be avoided by removing the . m+1 secure computation where However this is Thus by capturing the we are having an huge efficincy gain now that teh problem is reduced to antwo-party

\subsection{Protocols} \xh{This might go first with the algorithm box or figure.}
In this section, for each of the three entities we list down the interactions that are initiated by them.
\begin{itemize}\item CSP- The foremost duty of the CSP is to initialize the encryption scheme of Crypt$\epsilon$. Specifically the CSP generates the key pair $(sk,pk)$ for the labeled homomorphic encryption. It stores $sk$ with itself and makes $pk$ public. Note that since only the CSP has access to the secret key $sk$, it is the only entity capable of decryption in Crypt$\epsilon$.
\item Data owners- Recall that each data owner owns a single private record which he/she shares with the AS in the encrypted form as follows. First every data owner represents his/her record in its respective per attribute one-hot-encoding format. For example, if the database schema is given by  $D=<Age,Gender>$ then a data owner with the record $<30, Male>$ would firstly represent it as $\mathcal{E}(D)=<[\underbrace{0,\ldots,0}_{29},1,\underbrace{0,\ldots,0}_{70}],[1,0]>$. This is followed by an element-wise encryption of this record of per attribute one-hot-encodings using the pubic key $pk$. In our aforementioned example, we get $\mathbf{D}=<[\underbrace{Enc(0),\ldots}_{29},Enc(1),\underbrace{\ldots,Enc(0)}_{70}],[Enc(1),Enc(0)]>$. Finally the data owner sends this encrypted record to the AS. Note that this is the only interaction that a data owner ever participates in. All the  query answering are carried out by the AS and the CSP with the data owners being completely off line. \item AS - After receiving the encrypted records from each of the data owners, the AS first collates them into a single encrypted database $\mathbf{\tilde{D}}$. For any subsequent query answering, $\mathbf{\tilde{D}}$ is subjected it to a series of transformations most of which are carried out by the AS by itself. However since the CSP is the only entity capable of decryption, for getting any measurement (even noisy) in the clear the AS has to interact with it. There are precisely two types of interactions between the AS and the CSP \begin{enumerate}\item Yao's Garbled Circuit \item Decryption of encrypted noisy value\end{enumerate}\end{itemize}
\end{comment}


\eat{Yet another alternative implementation could have been to engage the $m$ data owners and the \textsf{AS} in a $m+1$ secure computation protocol. This approach has two disadvantages. Firstly, as the number of data owners grow, the communication and computation overheads of this $m+1$ secure computation protocol would get prohibitively high. Secondly, this violates our requirement of off-line data owners. Thus by introducing a separate entity in the form of the \textsf{CSP}, we factor out the onus of participating in a secure multi party computation from the data owners and capture their computation power in a secure protocol between just the \textsf{CSP} and the \textsf{AS} instead %. Note that with the \textsf{CSP} in the picture, the secure computation is now reduced to a two-party case
irrespective of the number of data owners. %Not only does this improve the efficiency of our protocols drastically but is also advantageous from the perspective of ease of system implementation and maintenance. It is so because otherwise we would have had to maintain secure channels between all pairs of data owners, which would become extremely cumbersome with large values of $m$. Moreover all the data owners would have to be online for every program execution. Hence the choice of having a separate server in the form of the \textsf{CSP} is made from the efficiency point of view.
%The second assumption of an computationally bounded adversary is inherent in semantically secure cryptographic protocols. %Another design choice for Crypt$\epsilon$ could have been to keep the data owners in the loop for every program execution such that some of the data transformations could be pushed down to them. Since the data owners can perform the transformations on the plain text and in parallel, this could potentially improve performance. However this would require the data owners to be on-line during the program execution which might be unwieldy in practice especially with a large number of geographically dispersed data owners. 
\par %Keeping the efficiency of our implementation in mind, we used only two instances of simple two-party Yao's garbled circuits for Crypt$\epsilon$. In addition, we propose two optimizations that leverage on the fact that the \textsf{AS} is satisfied with differentially private outputs; this allows  us to expend some of the privacy budget in differentially private pre-processing of the encrypted data. 
The class of programs supported by Crypt$\epsilon$ is any program that can be expressed as a composition of  Crypt$\epsilon$ primitives followed by arbitrary post-processing. Crypt$\epsilon$ supports 7 transformation primitives and 2 measurement primitives. The noisy measurements allowed are the Laplace mechanism and the Noisy max (see section 4.2), two of the most popular and standard differentially private algorithms. The main constraint behind the design of the transformation primitives is that their composition should allow seamless sensitivity analysis.  Sensitivity analysis of arbitrary relational algebraic queries is a hard problem, for e.g. sensitivity of conjunctive counting queries with join operator is unbounded \cite{sensitivity}. Hence all the transformations that Crypt$\epsilon$ supports have bounded stability \cite{PINQ} such that the sensitivity analysis of any program written using them is straightforward. In fact, we showcase that the proposed Crypt$\epsilon$ primitives are indeed very powerful, enabling us to answer practically useful queries, such as linear counting queries etc. 
\\ 
}





\subsection{Trust Model}\label{sec:trust}
Both the servers, \textsf{AS} and \textsf{CSP} are completely untrusted in Crypt$\epsilon$. 
Thus from the data owners perspective the trust assumption is similar to that of \textsf{LDP}; the data owners need not place their trust in any external entity. 
However there are two modest differences in the Crypt$\epsilon$ setting from that of \textsf{LDP}.\\
 (1) We assume that the \textsf{AS} and the \textsf{CSP} are non-colluding and follow the \emph{honest-but-curious} (or \textit{semi-honest}) adversary model. %That is, they always follow the instructions of the protocol faithfully but strive to learn extra information about the private records from the messages received during the execution of the protocol. 
 Moreover we assume that each data owner has a private channel with the \textsf{AS}. This is to prevent any third party (including the \textsf{CSP}) from eavesdropping. \\
 (2) The adversary is now reduced to a \textit{computationally bounded} one as opposed to the information theoretic one  in \textsf{LDP}.
 

 %\subsection{\system Security Sketch}

 
 
 
 
 \eat{In this paper we consider a
semi-honest adversary  $Adv$ (see section 3.4) who can corrupt any subset of the data owners, the data analyst and at most one of the two
servers. This captures our assumption that the two servers are non-colluding. Thus the requisite security definition should state that $Adv$ only learns the data of the corrupted data owners and the differentially private output but nothing else about the honest data owners. In other words, the view of the adversary $Adv$ should be \emph{computationally indistinguishable} from a truly differentially private protocol. 
Let $P$ be a program that is submitted by the data analyst to the protocol $\Pi$ and it is to be run on the data set $\mathcal{D}$ with the privacy parameter $\epsilon$. Thus based on our discussion on noise addition in sec 3.2, we define the ideal functionality $\mathcal{F}=(\mathcal{F}_1,\mathcal{F}_2)$ of the protocol $\Pi$ as follows. Let $\mathcal{F}^s$ be a sub-module of the ideal functionality $\mathcal{F}$ and let program $P$ be a composition of sub-programs $P^s_i, i \in [l]$, i.e., $P=P^s_l(\cdots (P^s_2(P^s_1(\cdot))$   such that the sub-program $P^s_i$ has a single additional instantiation of a DP mechanism (either Laplace or Noisy-Max) that is not present in the previous sub-program $P^s_{i-1}$. Every sub-program ends at a DP mechanism, any post-processing computation is carried over to the next sub-program. Any additional post-processing after the execution of the entire program, can be captured in $output^\Pi(P,\mathcal{D},\epsilon$  which denotes the published output of \system after running $P$.
\\If $P^s$ uses Laplace mechanism \cite{Dork}, then
\begin{gather} 
\mathcal{F}^s_1(P^s,\mathcal{D},\epsilon^s)=P^s(\mathcal{D})+\eta_2\\\mathcal{F}^s_2(P^s,\mathcal{D},\epsilon^s)=P^s(\mathcal{D})+\eta_1\\ \eta_1, \eta_2 \sim Lap(\frac{\Delta}{\epsilon^s})\end{gather}  where  $\Delta$  is the suitable sensitivity of $P^s$. In this case, $output^{\Pi}(P^s,\mathcal{D},\epsilon^s)$  is given by $f\big(P^s(\mathcal{D})+\eta_1+\eta_2\big)$ where $f(\cdot)$ is an arbitrary post-processing function. \\
If $P^s$ uses Noisy-Max mechanism \cite{Dork}, then
\begin{multline}
\mathcal{F}^s_1(P^s,\mathcal{D},\epsilon^s)=\mathcal{F}^s_2(P,\mathcal{D},\epsilon^s)=f\big(\textit{Noisy-Max}(P^s(\mathcal{D}),\Delta,\epsilon^s)\big) 
\end{multline} where $P^s(\mathcal{D})$ produces a vector and  $\Delta$ is the suitable sensitivity of the program. $output^{\Pi}(P^s,\mathcal{D},\epsilon^s)$ in this case is equal to \\ $f\big(\textit{Noisy-Max}(P^s(\mathcal{D}),\Delta,\epsilon^s)\big)$.  Thus, using the above equation, \begin{gather*}\mathcal{F}_1(P,\mathcal{D},\epsilon)=\mathcal{F}^{s,l}_1\Big(\cdots\mathcal{F}^{s,2}_1\big(\mathcal{F}_1^{s,1}(P^{s,1},\mathcal{D},\epsilon^1),P^{s,2},\mathcal{D},\epsilon^{2}\big)\\\cdots P^{s,l},\mathcal{D},\epsilon^l\Big) \numberthis \\\mathcal{F}_2(P,\mathcal{D},\epsilon)=\mathcal{F}^{s,l}_2\Big(\cdots\mathcal{F}^{s,2}_2\big(\mathcal{F}_2^{s,1}(P^{s,1},\mathcal{D},\epsilon^1),P^{s,2},\mathcal{D},\epsilon^{2}\big)\\\cdots P^{s,l},\mathcal{D},\epsilon^l\Big) \numberthis \\\epsilon=\sum_i^l\epsilon^i\end{gather*}By Theorem 1, $\mathcal{F}$ is $\epsilon$-DP.
Formally, using the standard simulation based definition \cite{Oded},
\begin{theorem}  Let $S \subset \{1,...,m\}$ then $\Pi$, (i.e. the protocol for an end-to-end program execution in \system) realizes $\mathcal{F}$ (eq 3-6)  with correctness and privacy against
the adversaries $Adv_1=\textsf{AS} \cup \{\textsf{DO}_i, i \in S\} \cup \mbox{Data Analyst}$  and $Adv_2=\textsf{CSP} \cup  \{ \textsf{DO}_i, i \in S\} \cup \mbox{Data Analyst}$
 if there exists  P.P.T algorithms $Sim_1$ and $Sim_2$ such that  \begin{align*}
 \big\{Sim_1({D_i, i \in S},\mathcal{F}_1(P,\mathcal{D},\epsilon)),\mathcal{F}(P,\mathcal{D},\epsilon)\big\} &\\\stackrel{C}{\equiv} \big\{view^{\Pi}_{Adv1}(P,\mathcal{D},\epsilon),output^{\Pi}(P,\mathcal{D},\epsilon)\big\}  \numberthis\label{adv1}
               \\
 \big\{Sim_2({D_i, i \in S},\mathcal{F}_2(P,\mathcal{D},\epsilon)),\mathcal{F}(P,\mathcal{D},\epsilon))\big\} &\\\stackrel{C}{\equiv}\big\{ view^{\Pi}_{Adv2}(P,\mathcal{D},\epsilon),output^{\Pi}(P,\mathcal{D},\epsilon)\big\}  \numberthis\label{adv2}
\end{align*} for all possible inputs  where $ \stackrel{C}{\equiv}$ denotes computational indistinguishability and $view^{\Pi}_i$ denotes the view of entity $i$ in protocol $\Pi$. 
\end{theorem}}











\eat{Here we just present an intuitive understanding of it. The interactions between the \textsf{AS} and the \textsf{CSP} can be categorised as \\(1) \textsf{CSP} generates garbled circuits with noisy outputs that are evaluated by the \textsf{AS}\\(2) \textsf{AS} sends encrypted masked data to the \textsf{CSP} and gets a transformed encrypted data in response \\(3)\textsf{AS} sends encrypted noisy data and gets back the data in the cleat with additional noise from the \textsf{CSP}\\
The garbled circuits are inherently semantically secure. For the second type of interaction, the random
mask hides the true plaintext
from the \textsf{CSP} while the \textsf{AS} cannot decrypt anything as it does not have access to the secret key $sk$. The last type of interaction outputs a noisy measurement over the data and illustrates the fact that both  \textsf{AS} and \textsf{CSP} add noise to the final answer in \system to ensure that both the servers are allowed only a differentially private  view of the data. Moreover, in
addition to the \emph{Program Executor} module of the \textsf{AS}, the data analyst
communicates the \system program and the privacy parameter $\epsilon$
to the \textit{Privacy Engine} module of the \textsf{CSP}. This enables the \textsf{CSP} to
compute the sensitivity of the program for itself (required while
adding its own noise) thereby thwarting any privacy budget over
expenditure attempts.}
 




\subsection{Discussion}\label{sec:discuss-arch}
 Crypt$\epsilon$  is based on the premise that there are $m$  data owners, each possessing a private data record, and the \textsf{AS} is the primary entity who is interested in learning certain differentially private statistics on the collective data.  Thus in \system, we require the \textsf{AS} to  shoulder the major chunk of the workload for any Crypt$\epsilon$ program execution; interactions with the \textsf{CSP} should be minimal and only related to data decryption.
Keeping this in  mind, we design the \textsf{AS} to perform most of the data transformations by itself (Table \ref{perf}). Specifically for every Crypt$\epsilon$ program, the \textsf{AS} processes the whole database and transforms it into concise representations (like an encrypted scalar or a short vector) which is then decrypted with the help of the \textsf{CSP}. It is interesting to note that we could have had an alternative implementation for Crypt$\epsilon$ where the private database is equally shared between the two servers and they engage in a secret share based secure computation protocol for computing the differentially private answers. However, this would require both the servers to do almost equal amount of work for every program. Such an arrangement would be justified only if both the servers are equally invested in learning the differentially private statistics and is ill-suited for Crypt$\epsilon$. Additionally, a secret-share based computation would be much more communication intensive resulting in a performance hit. 

The primitives for \system have been designed bearing two things in mind. Firstly, their composition should allow easy sensitivity analysis (for e.g. transformations must have bounded stability). Secondly, all the primitives should have very efficient implementations. Thus although the architecture of \system imposes no fundamental restriction on its expressibility and in theory we can enjoy the same algorithmic power as that of \textsf{CDP}, we restrict the expressibility in the current implementation of \system to ensure practicality of \system programs. Nevertheless, there is a separation between \system and \textsf{LDP} as explained in Appendix D2.


\eat{\begin{table}[h!]
\small
\centering
\caption {Comparative analysis of the different DP models}
 \begin{tabular}{l| c c c}  \toprule
\multicolumn{1}{c}{\textbf{Features}} & \textbf{LDP}  & \textbf{CDP}  & \textbf{Crypt$\epsilon$}  \\ [0.5ex] 
 \midrule \midrule \# Servers & 1& 1 & 2\\\hline
Trust  & & & Untrusted \\  Assumption & Untrusted & Trusted & Semi Honest \\for Server &  &   &  Non-Colluding  \\ \hline
Data Storage & \multirow{2}{*}{Noisy} & \multirow{2}{*}{Clear} & \multirow{2}{*}{Encrypted} \\in Server & &  &  \\\hline
Adversary & Unbounded & Unbounded & Bounded \\\hline
 Error & $O\Big(\frac{\sqrt(n)}{\epsilon}\Big)$& $O\Big(\frac{1}{\epsilon}\Big)$ & $O\Big(\frac{1}{\epsilon}\Big)$\\\hline
 Impossibility & Everything && \\results & beyond SQ model & None & None\footnotemark\\
  [1ex] 
 \bottomrule
 \end{tabular}
\end{table}
\footnotetext{Theoretically no restriction, however practical constraints maybe present}}

%\arc{ Can add another column for Mixnets maybe?}

